A new feedback cycle in the archetypal cooling flow group NGC 5044

The fate of cooling gas in the centers of galaxy clusters and groups is still not well understood, as is also the case for the complex process of triggering active galactic nucleus (AGN) outbursts in their central dominant galaxies, and the consequent re-heating of the gas by the AGN jets. With the largest known reservoir of cold molecular gas of any group-dominant galaxy and three epochs of AGN activity visible as cavities in its hot gas, NGC 5044 is an ideal system in which to study the cooling/AGN feedback cycle at the group scale. We present VLBA observations of NGC 5044 to ascertain the current state of the central AGN. We find a compact core and two small jets aligned almost in the plane of the sky, and in the orthogonal direction to the location of cavities. We construct the radio/sub-mm spectral energy distribution (SED) over more than three orders of magnitude. We find that below 5 GHz the spectrum is best fit by a self-absorbed continuous injection model representing emission coming from the jets, while the higher frequencies show clear signs of an advection dominated accretion flow. We derive a black hole mass and accretion rate consistent with independent measurements. We conclude that the age of the jets is much younger than the innermost cavities, marking the start of a new feedback cycle.

==> table_obslog.tex <==
%***********************
%-----TABLE--1----------
\begin{deluxetable*}{ccccc}
 \tablecaption{VLBA observing log for project BS283}
 \tablehead{
 \colhead{Observation} &
 \colhead{A1} &
 \colhead{A2} &
 \colhead{B1} & 
 \colhead{B2} 
 }
\startdata
Date & 2020/03/13 & 2020/03/19 & 2020/03/20 & 2020/04/13 \\
Frequency (GHz) & 5 & 5 & 8.5 & 8.5 \\
Time (min) & & & & \\
Beam size ($\si{mas} \times \si{mas}$) & & & & \\
Beam size (pc$\times$pc) & & & & \\
rms ($\si{\mu Jy\,bm^{-1}}$) & & & & \\
Comment & 9\% downtime due  & 0.2\% downtime due  & 1\% downtime,  & 0\% downtime\\
 & to winds at KP & to winds at KP & high $T_\textrm{sys}$ at NL & \\
\enddata
\tablecomments{Observation date, representative frequency, bandpass calibrator, on target science integration time, restoring beam, rms sensitivity. Bandpass calibrator was J0927+0329 and the phase reference source was 1314-134 for all observations.  \label{tab:obslog}}
\end{deluxetable*}
